Transducers with origin information

Call a string-to-string transducer regular if it can be realised by one of the following equivalent models: mso transductions, two-way deterministic automata with output, and streaming transducers with registers. This paper proposes to treat origin information as part of the semantics of a regular string-to-string transducer. With such semantics, the model admits a machine-independent characterisation, Angluin-style learning in polynomial time, as well as effective characterisations of natural subclasses such as one-way transducers or first-order definable transducers.

==> equivalence.tex <==
	
	\subsection{Equivalence}
	
	
	
	\begin{theorem}\label{thm:}
		The following problem is co-NP complete.
		\begin{itemize}
			\item Input: two streaming look-ahead transducers.
			\item Question: are they equivalent as transducers with origin information?
		\end{itemize}
	\end{theorem}
	\begin{pr}
		\paragraph*{Hardness.} The lower bound is a reduction from the following problem: given several regular languages  over the same alphabet,  decide if their union is all colours. This problem is PSPACE complete, already when the languages are given by deterministic automata.
		
		Suppose that we have an input instance consisting of $n$ automata. We want to decide if every colours is accepted by at least one of them.  Suppose that $Q_i$ is the state space of the $i$-th automaton. We design a transducer  $f$, whose  registers are the disjoint union of all $Q_i$, with the following property. For every $i \in \set{1,\ldots,n}$, after reading  a colour $w$, the unique nonempty register in $Q_i$ is the one that corresponds to  the state of $i$-th automaton after reading $w$. This register update of this transducer simply mirrors the transition function of the automata: when reading a letter $a$, it does the following operations in parallel for every state $q$ in every set $Q_i$:
		\begin{quote}
			Into register $q$, put the concatenation (in some arbitrary order) of the values of all registers that correspond to states which are mapped into $q$ by the transition function of the $i$-th automaton over letter $a$.
		\end{quote}
		A special update is required for the first letter of the input, which ensures that a nonempty colour is placed into the register corresponding to the states of the automata after reading this first letter. 		
		What is important about $f$  is that its size polynomial in the combined size of the automata in the problem instance: its registers are the combined state spaces of the automata, it has two control states (for the first letter and the other letters), and its register update function is of the same size as the combined transition tables of the automata.
		
		From the transducer $f$ we construct a new transducer $f'$, whose alphabet is the same as the input alphabet of $f$, plus a new symbol $\#$. When the transducer reads  $\#$, it outputs the contents of all registers that correspond to accepting states.
		
		
		for each state $q$ it appends the contents of regiser $q$ to the end 
		
		For each language, let 
		
		Consider a formula 
		\begin{align*}
			\varphi = \varphi_1 \land \cdots \land \varphi_n
		\end{align*}
		in CNF. We construct a transducer $f_\varphi$ with input alphabet $\set{0,1}$ and output alphabet $\set{a}$ as follows.  such that 
		\begin{align*}
			f(\underline{x_1 \cdots x_n} | 0 | \underline 0) = \begin{cases}
				\leftvar\ & \mbox{if $\varphi(x_1,\ldots,x_n)$}\\
				\leftvar\ \rightvar\ \leftvar & \mbox{otherwise}\\
			\end{cases}
		\end{align*}
		Suppose that $\varphi$ is a conjuction
		The transducer has one register for every 
		
		
		We first observe that a  string-to-string function $f$ with origin information is uniquely determinied by the function
		\begin{equation}
			\label{eq:the-triple-function}
(x,y,z) \qquad \mapsto \qquad			f(\underline x | a | \underline y)
		\end{equation}
		where $x$ and $y$ are strings and $a$ is a letter. This is because 
				\begin{align*}
			f(|a_1 \cdots a_n | ) = x_1 \otimes \cdots \otimes x_n \qquad \mbox{where }x_i =  f(\underline{a_1 \cdots a_{i-1}}|a_i|\underline{a_{i+1}\cdots a_n}),
		\end{align*}
		which can be shown by induction on $n$. Therefore, in order two test equivalence of two lookahead transducers, it remains to test if they induce the same maps as in equation~\eqref{eq:the-triple-function}. 
	\end{pr}
	
	The above


	

==> provenance.tex <==
\section{Provenance}

\begin{theorem}
	The following define the same classes of colour-to-colour functions with provenance:
	\begin{enumerate}
		\item lookahead transducers;
		\item two-way deterministic automata with output;
		\item MSO transductions.
	\end{enumerate}
	
\end{theorem}

